RoboCup@Home: Summarizing achievements in over eleven years of competition

Scientific competitions are important in robotics because they foster knowledge exchange and allow teams to test their research in unstandardized scenarios and compare result. In the field of service robotics its role becomes crucial. Competitions like RoboCup@Home bring robots to people, a fundamental step to integrate them into society. In this paper we summarize and discuss the differences between the achievements claimed by teams in their team description papers, and the results observed during the competition^1 from a qualitative perspective. We conclude with a set of important challenges to be conquered first in order to take robots to people's homes. We believe that competitions are also an excellent opportunity to collect data of direct and unbiased interactions for further research. ^1 The authors belong to several teams who have participated in RoboCup@Home as early as 2007

==> Makefile <==
PREFIX  = paper

TEXFILE = $(PREFIX).tex
AUXFILE = $(PREFIX).aux
PDFFILE = $(PREFIX).pdf
SILENT  = @

TEMP	= *.aux *.bbl *.blg *.log *.out *.tmp *.synctex.gz
RMFILES = $(TEMP) *~ *.toc *.idx *.ilg *.ind *.log *.lot *.lof \
          *.adx *.and *.abb *.ldx .temp* *.tar mergedfile.pdf


all:
	$(SILENT) make -s clean
#	$(SILENT) rubber --pdf --force $(TEXFILE)
	$(SILENT) rubber --pdf --force $(TEXFILE)
#	$(SILENT) rubber --clean $(wildcard *.tex)
#	$(SILENT) pdftk $(PDFFILE) CopyrightReceipt.pdf cat output mergedfile.pdf
#	$(SILENT) cp -f mergedfile.pdf $(PDFFILE)
#	$(SILENT) rm mergedfile.pdf
#	$(SILENT) rm -rf $(TEMP)


clean:
	$(SILENT) rubber --clean $(wildcard *.tex)
	$(SILENT) rm -rf $(TEMP)
	$(SILENT) rm -f $(RMFILES)

